Extending the planar theory of anyons to quantum wire networks

The braiding of the worldlines of particles restricted to move on a network (graph) is governed by the graph braid group, which can be strikingly different from the standard braid group known from two-dimensional physics. It has been recently shown that imposing the compatibility of graph braiding with anyon fusion for anyons exchanging at a single wire junction leads to new types of anyon models with the braiding exchange operators stemming from solutions of certain generalised hexagon equations. In this work, we establish these graph-braided anyon fusion models for general wire networks. We show that the character of braiding strongly depends on the graph-theoretic connectivity of the given network. In particular, we prove that triconnected networks yield the same braiding exchange operators as the planar anyon models. In contrast, modular biconnected networks support independent braiding exchange operators in different modules. Consequently, such modular networks may lead to more efficient topological quantum computer circuits. Finally, we conjecture that the graph-braided anyon fusion models will possess the (generalised) coherence property where certain polygon equations determine the braiding exchange operators for an arbitrary number of anyons. We also extensively study solutions to these polygon equations for chosen low-rank multiplicity-free fusion rings, including the Ising theory, quantum double of Z2, and Tambara-Yamagami models. We find numerous solutions that do not appear in the planar theory of anyons.

==> Tables/LollipopSolutionsTab.tex <==
\begin{tabular}{>{\raggedright}m{2cm}>{\centering}m{1.6cm}>{\centering}m{1.6cm}>{\centering}m{2cm}>{\centering}m{2cm}>{\centering}m{3cm}}
\hline
\noalign{\vskip1mm}
\multirow{2}{2cm}{Ring} & \multicolumn{5}{c}{Amount of solutions per type of equations (3 particles)}\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6}
\noalign{\vskip1mm}
 & Planar Hexagon & Circle & Lollipop Trijunction & Full Lollipop & Lollipop but

non-planar\tabularnewline
\hline
\hline
\multirow{2}{2cm}{$\mathbb{\mathbb{Z}}_{2}$} & $2$ & $2^{2}$ & $2$ & $2^{3}$ & $0$\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6}
\noalign{\vskip1mm}
 & $2$ & $2^{2}$ & $2$ & $2^{3}$ & $0$\tabularnewline
\noalign{\vskip1mm}
\hline
Fibonacci & $2$ & $2$ & $2$ & $2^{2}$ & $0$\tabularnewline
\noalign{\vskip1mm}
\hline
\multirow{2}{2cm}{Ising} & $2^{2}$ & $2^{4}$ & $2^{2}$ & $2^{6}$ & $0$\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6}
\noalign{\vskip1mm}
 & $2^{2}$ & $2^{4}$ & $2^{2}$ & $2^{6}$ & $0$\tabularnewline
\noalign{\vskip1mm}
\hline
\multirow{3}{2cm}{Rep($D_{3}$)} & $3$ & $3$ & $3$ & $3^{2}$ & $0$\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6}
\noalign{\vskip1mm}
 & $0$ & $3$ & $0$ & $0$ & $0$\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6}
\noalign{\vskip1mm}
 & $0$ & $3$ & $0$ & $0$ & $0$\tabularnewline
\noalign{\vskip1mm}
\hline
\multirow{3}{2cm}{$\mathbb{\mathbb{Z}}_{3}$} & $3$ & $3^{3}$ & $3^{2}$ & $3^{5}$ & $(3-1)3^{4}$\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6}
\noalign{\vskip1mm}
 & $0$ & $3^{3}$ & $3^{2}$ & $3^{5}$ & $3^{5}$\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6}
\noalign{\vskip1mm}
 & $0$ & $3^{3}$ & $3^{2}$ & $3^{5}$ & $3^{5}$\tabularnewline
\noalign{\vskip1mm}
\hline
\multirow{8}{2cm}{$\mathbb{\mathbb{Z}}_{2}\times\mathbb{\mathbb{Z}}_{2}$} & $2^{4}$ & $2^{8}$ & $2^{6}$ & $2^{14}$ & $(2^{2}-1)2^{12}$\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6}
\noalign{\vskip1mm}
 & $2^{4}$ & $2^{8}$ & $2^{6}$ & $2^{14}$ & $(2^{2}-1)2^{12}$\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6}
\noalign{\vskip1mm}
 & $0$ & $2^{8}$ & $2^{6}$ & $2^{14}$ & $2^{14}$\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6}
\noalign{\vskip1mm}
 & $0$ & $2^{8}$ & $2^{6}$ & $2^{14}$ & $2^{14}$\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6}
\noalign{\vskip1mm}
 & $2^{4}$ & $2^{8}$ & $2^{6}$ & $2^{14}$ & $(2^{2}-1)2^{12}$\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6}
\noalign{\vskip1mm}
 & $2^{4}$ & $2^{8}$ & $2^{6}$ & $2^{14}$ & $(2^{2}-1)2^{12}$\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6}
\noalign{\vskip1mm}
 & $0$ & $2^{8}$ & $2^{6}$ & $2^{14}$ & $2^{14}$\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6}
\noalign{\vskip1mm}
 & $0$ & $2^{8}$ & $2^{6}$ & $2^{14}$ & $2^{14}$\tabularnewline
\noalign{\vskip1mm}
\hline
\multirow{4}{2cm}{$\mathbb{\mathbb{Z}}_{4}$} & $2^{2}$ & $2^{8}$ & $2^{6}$ & $2^{14}$ & $(2^{2}-1)(2^{3}-3)2^{10}$\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6}
\noalign{\vskip1mm}
 & $0$ & $2^{8}$ & $2^{6}$ & $2^{14}$ & $2^{14}$\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6}
\noalign{\vskip1mm}
 & $2^{2}$ & $2^{8}$ & $2^{6}$ & $2^{14}$ & $(2^{2}-1)(2^{3}-3)2^{10}$\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6}
\noalign{\vskip1mm}
 & $0$ & $2^{8}$ & $2^{6}$ & $2^{14}$ & $2^{14}$\tabularnewline
\noalign{\vskip1mm}
\hline
\multirow{8}{2cm}{Rep($D_{4}$)} & $2^{3}$ & $2^{7}$ & $2^{3}$ & $2^{10}$ & $0$\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6}
\noalign{\vskip1mm}
 & $2^{3}$ & $2^{7}$ & $2^{3}$ & $2^{10}$ & $0$\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6}
\noalign{\vskip1mm}
 & $2^{3}$ & $2^{7}$ & $2^{3}$ & $2^{10}$ & $0$\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6}
\noalign{\vskip1mm}
 & $2^{3}$ & $2^{7}$ & $2^{3}$ & $2^{10}$ & $0$\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6}
\noalign{\vskip1mm}
 & $2^{3}$ & $2^{7}$ & $2^{3}$ & $2^{10}$ & $0$\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6}
\noalign{\vskip1mm}
 & $2^{3}$ & $2^{7}$ & $2^{3}$ & $2^{10}$ & $0$\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6}
\noalign{\vskip1mm}
 & $2^{3}$ & $2^{7}$ & $2^{3}$ & $2^{10}$ & $0$\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6}
\noalign{\vskip1mm}
 & $2^{3}$ & $2^{7}$ & $2^{3}$ & $2^{10}$ & $0$\tabularnewline
\hline
\noalign{\vskip1mm}
\end{tabular}


==> Tables/TrijunctionSolutionsTab.tex <==
\begin{tabular}{|>{\raggedright}p{1.7cm}|>{\raggedright}m{1.7cm}|>{\raggedright}m{2.7cm}|>{\raggedright}m{1.7cm}|>{\raggedright}m{2.7cm}|>{\raggedright}m{1.7cm}|}
\hline
\multirow{3}{1.7cm}{\textbf{Ring}} & \multicolumn{5}{c|}{\textbf{Solutions to Trijunction}}\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6}
 & \multicolumn{2}{c|}{$N=3$} & \multicolumn{3}{c|}{$N=4$}\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6}
 & \textbf{Amount} & \textbf{Free Variables} & \textbf{Amount} & \textbf{Free Variables} & \textbf{Planar?}\tabularnewline
\hline
\multirow{2}{1.7cm}{$\mathbb{\mathbb{Z}}_{2}$} & $1$ & \multirow{2}{2.7cm}{All nontrivial $R$ symbols} & $1$ & \multirow{2}{2.7cm}{All nontrivial $R$ symbols} & UCC\tabularnewline
\cline{2-2} \cline{4-4} \cline{6-6}
 & $1$ &  & $1$ &  & UCC\tabularnewline
\hline
\multirow{1}{1.7cm}{Fibonacci} & $2$ & \multirow{1}{2.7cm}{$0$} & \multirow{1}{1.7cm}{$2$} & $0$ & Always\tabularnewline
\hline
\multirow{4}{1.7cm}{Ising} & $1$ & $2$ & $1$ & $1$ & UCC\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6}
 & $1$ & $2$ & $1$ & $1$ & UCC\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6}
 & $1$ & $2$ & $1$ & $1$ & UCC\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6}
 & $1$ & $2$ & $1$ & $1$ & UCC\tabularnewline
\hline
\multirow{3}{1.7cm}{Rep($D_{3}$)} & $1$ & $2$ & $3$ & 0 & Always\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6}
 & $0$ & / & $0$ & / & /\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6}
 & $0$ & / & $0$ & / & /\tabularnewline
\hline
\multirow{3}{1.7cm}{$\mathbb{\mathbb{Z}}_{3}$} & $1$ & \multirow{3}{2.7cm}{All nontrivial $R$ symbols} & $1$ & \multirow{3}{2.7cm}{All nontrivial $R$ symbols} & UCC\tabularnewline
\cline{2-2} \cline{4-4} \cline{6-6}
 & $1$ &  & $1$ &  & Never\tabularnewline
\cline{2-2} \cline{4-4} \cline{6-6}
 & $1$ &  & $1$ &  & Never\tabularnewline
\hline
\multirow{8}{1.7cm}{$\mathbb{\mathbb{Z}}_{2}\times\mathbb{\mathbb{Z}}_{2}$} & $1$ & \multirow{8}{2.7cm}{All nontrivial $R$ symbols} & $1$ & \multirow{8}{2.7cm}{All nontrivial $R$ symbols} & UCC\tabularnewline
\cline{2-2} \cline{4-4} \cline{6-6}
 & $1$ &  & $1$ &  & UCC\tabularnewline
\cline{2-2} \cline{4-4} \cline{6-6}
 & $1$ &  & $1$ &  & Never\tabularnewline
\cline{2-2} \cline{4-4} \cline{6-6}
 & $1$ &  & $1$ &  & Never\tabularnewline
\cline{2-2} \cline{4-4} \cline{6-6}
 & $1$ &  & $1$ &  & UCC\tabularnewline
\cline{2-2} \cline{4-4} \cline{6-6}
 & $1$ &  & $1$ &  & UCC\tabularnewline
\cline{2-2} \cline{4-4} \cline{6-6}
 & $1$ &  & $1$ &  & Never\tabularnewline
\cline{2-2} \cline{4-4} \cline{6-6}
 & $1$ &  & $1$ &  & Never\tabularnewline
\hline
\multirow{4}{1.7cm}{$\mathbb{\mathbb{Z}}_{4}$} & $1$ & \multirow{4}{2.7cm}{All nontrivial $R$ symbols} & $1$ & \multirow{4}{2.7cm}{All nontrivial $R$ symbols} & UCC\tabularnewline
\cline{2-2} \cline{4-4} \cline{6-6}
 & $1$ &  & $1$ &  & Never\tabularnewline
\cline{2-2} \cline{4-4} \cline{6-6}
 & $1$ &  & $1$ &  & UCC\tabularnewline
\cline{2-2} \cline{4-4} \cline{6-6}
 & $1$ &  & $1$ &  & Never\tabularnewline
\hline
\multirow{8}{1.7cm}{Rep($D_{4}$)} & $4$ & $10$ & $4$ & $1$ & UCC\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6}
 & $4$ & $10$ & $4$ & $1$ & UCC\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6}
 & $4$ & $10$ & $4$ & $1$ & UCC\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6}
 & $4$ & $10$ & $4$ & $1$ & UCC\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6}
 & $4$ & $10$ & $4$ & $1$ & UCC\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6}
 & $4$ & $10$ & $4$ & $1$ & UCC\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6}
 & $4$ & $10$ & $4$ & $1$ & UCC\tabularnewline
\cline{2-6} \cline{3-6} \cline{4-6} \cline{5-6} \cline{6-6}
 & $4$ & $10$ & $4$ & $1$ & UCC\tabularnewline
\hline
\end{tabular}

